Towards Interpreting BERT for Reading Comprehension Based QA

BERT and its variants have achieved state-of-the-art performance in various NLP tasks. Since then, various works have been proposed to analyze the linguistic information being captured in BERT. However, the current works do not provide an insight into how BERT is able to achieve near human-level performance on the task of Reading Comprehension based Question Answering. In this work, we attempt to interpret BERT for RCQA. Since BERT layers do not have predefined roles, we define a layer's role or functionality using Integrated Gradients. Based on the defined roles, we perform a preliminary analysis across all layers. We observed that the initial layers focus on query-passage interaction, whereas later layers focus more on contextual understanding and enhancing the answer prediction. Specifically for quantifier questions (how much/how many), we notice that BERT focuses on confusing words (i.e., on other numerical quantities in the passage) in the later layers, but still manages to predict the answer correctly. The fine-tuning and analysis scripts will be publicly available at https://github.com/iitmnlp/BERT-Analysis-RCQA .

==> semantic_stats.tex <==
% % Please add the following required packages to your document preamble:
% % \usepackage{multirow}
% % \usepackage{graphicx}
% \begin{table*}[]
% \centering
% \resizebox{\textwidth}{!}{%
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \textbf{Model} & \textbf{Layer Name} & \textbf{\% entities} & \textbf{\% verbs} & \textbf{\% stop words} & \textbf{\% adverbs} & \textbf{\% punct marks} & \textbf{\begin{tabular}[c]{@{}c@{}}\% entities in\\ answer span\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\% entities not \\ in answer span\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}\% words in \\ answer span\end{tabular}} & \textbf{Q-words} & \textbf{\begin{tabular}[c]{@{}c@{}}Contextual\\ Words\end{tabular}} \\ \hline
% \multirow{12}{*}{BERT} & Layer 0 & 61.21 & 12.92 & 12.63 & 2.73 & 11.41 & 19.25 & 7.74 & 26.99 & 22.94 & 26.28 \\ \cline{2-12} 
%  & Layer 1 & 65.09 & 13.81 & 10.71 & 3.13 & 8.27 & 19.66 & 6.43 & 26.09 & 24.35 & 25.68 \\ \cline{2-12} 
%  & Layer 2 & 64.68 & 14.19 & 13.71 & 3.24 & 5.25 & 21.82 & 8.08 & 29.9 & 22.41 & 29.94 \\ \cline{2-12} 
%  & Layer 3 & 60.59 & 12.98 & 16.27 & 2.76 & 8.52 & 21.73 & 8.72 & 30.44 & 19.55 & 29.5 \\ \cline{2-12} 
%  & Layer 4 & 58.57 & 12.32 & 19.93 & 2.87 & 7.29 & 21.1 & 8.96 & 30.06 & 18.33 & 28.96 \\ \cline{2-12} 
%  & Layer 5 & 56.52 & 12.34 & 19.35 & 2.73 & 10.29 & 21.7 & 9.05 & 30.75 & 14.71 & 29.95 \\ \cline{2-12} 
%  & Layer 6 & 59.36 & 12.13 & 17.38 & 2.51 & 9.75 & 22.64 & 8.61 & 31.25 & 15.33 & 31.0 \\ \cline{2-12} 
%  & Layer 7 & 60.3 & 11.31 & 16.23 & 2.61 & 10.85 & 23.27 & 9.1 & 32.37 & 12.29 & 32.08 \\ \cline{2-12} 
%  & Layer 8 & 65.44 & 11.59 & 14.59 & 2.58 & 6.94 & 22.69 & 8.1 & 30.78 & 18.91 & 31.04 \\ \cline{2-12} 
%  & Layer 9 & 64.1 & 10.11 & 12.98 & 2.42 & 11.82 & 25.58 & 9.0 & 34.58 & 10.21 & 34.83 \\ \cline{2-12} 
%  & Layer 10 & 68.73 & 8.67 & 12.2 & 2.11 & 9.64 & 25.88 & 8.43 & 34.31 & 10.56 & 34.73 \\ \cline{2-12} 
%  & Layer 11 & 65.02 & 8.77 & 14.57 & 2.31 & 10.63 & 25.6 & 9.03 & 34.63 & 12.0 & 34.93 \\ \hline
% \end{tabular}%
% }
% \caption{Semantic statistics about top-5 words}
% \label{tab:semantic_stats}
% \end{table*}
% Please add the following required packages to your document preamble:
% \usepackage{graphicx}
\begin{table}
\centering
\resizebox{0.85\linewidth}{!}{%
\begin{tabular}{|c|c|c|c|}
\hline
\textbf{Layer Name} & \textbf{\begin{tabular}[c]{@{}c@{}}\% answer\\ span\end{tabular}} & \textbf{\% Q-words} & \textbf{\begin{tabular}[c]{@{}c@{}}\% Contextual\\ Words\end{tabular}} \\ \hline \hline
Layer 0 & 26.99 & 22.94 & 9.45 \\ \hline
Layer 1 & 26.09 & 24.35 & 9.43 \\ \hline
Layer 2 & 29.9 & 22.41 & 11.65 \\ \hline
Layer 3 & 30.44 & 19.55 & 11.13 \\ \hline
Layer 4 & 30.06 & 18.33 & 11.23 \\ \hline
Layer 5 & 30.75 & 14.71 & 11.57 \\ \hline
Layer 6 & 31.25 & 15.33 & 11.94 \\ \hline
Layer 7 & 32.37 & 12.29 & 12.32 \\ \hline
Layer 8 & 30.78 & 18.91 & 12.07 \\ \hline
Layer 9 & 34.58 & 10.21 & 13.41 \\ \hline
Layer 10 & 34.31 & 10.56 & 13.39 \\ \hline
Layer 11 & 34.63 & 12.0 & 13.74 \\ \hline
\end{tabular}%
}
\caption{Semantic statistics of top-5 words - SQuAD}
\label{tab:semantic_stats_squad}
\end{table}


==> tsne.tex <==
\input{emnlp2020-templates/example_squad}
\begin{figure}
    \centering
    \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{emnlp2020-templates/tsne-plots/tsne_qn_31_layer_0.png} 
        % \caption{}
        % \label{bert_layer0}
    \end{subfigure}
     \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{emnlp2020-templates/tsne-plots/tsne_qn_31_layer_5.png} 
        % \caption{}
        % \label{bert_layer5}
    \end{subfigure} 
    \caption{tSNE plots for Layers 0 and 5 to analyse how the word representations evolve across layers.}
    \label{fig:tsne}
\end{figure}

\begin{figure} %\ContinuedFloat
    \centering
     \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{emnlp2020-templates/tsne-plots/tsne_qn_31_layer_8.png} 
        % \caption{}
        % \label{bert_layer8}
    \end{subfigure}
     \begin{subfigure}{0.4\textwidth}
        \centering
        \includegraphics[width=\textwidth]{emnlp2020-templates/wordemb_tsne_qn31/bert_perp40/tsne_qn_31_layer_11.png} 
        % \caption{}
        % \label{bert_layer11}
    \end{subfigure} 
    \caption{tSNE plots across Layers 8 and 11 to analyse how the word representations evolve across layers.}
    \label{fig:tsne2}
\end{figure}



%\section{Qualitative Analysis on learnt representations at each layer}
%We carefully analyze how word representations evolve across layers few {passage, question, answer} triplets. We present one such example in Table \ref{fig:tsne}. We divided the passage words into three categories: answer span, support words (words around the answer span) and special tokens. We then retrieve the t-sne plots for word representations for all layers. Note that the other words in the passage have been grayed out. We observe that in Layer 0, all the words in the passage are very similar to each other. From Layer 2 onwards, it cluster entities, and answer types together. 
%From Table \ref{fig:tsne} (row 1), we can infer that for DCN the change in word-representations across layers is more streamlined/intuitive. In the word-embedding layer, words with similar syntactic meanings are closer on the t-SNE plot. In the contextual layer, most of the words get nearer to their semantically closer context on the t-SNE plot. However, as a result, in the example(Question 2 in Table \ref{tab:run_exp}), the correct answer ``eight" comes close to the syntactically correct answer ``four" thereby making both of them equally likely to get predicted. We see that in the cross-interaction layer, the model is able to make that distinction. The answer-words, relevant-words, and question-words come closer as compared to their distance with other words. 

%For BERT (Table \ref{fig:tsne}, (row 2)), since the role of the 12 different layers is not predefined, we try to draw a parallel between some layers which seem to capture contextual and query-passage relationship, with the corresponding ones in DCN. However, we observe that the information flow is not as streamlined/intuitive as in DCN; for instance, the representation learned from layer $7$,  was not carried forward to the subsequent layers. This observation is similar for the first two t-SNE plots for BERT, although, the answer, the relevant-words, and the question words appear to be much closer. The layer $7$, which seems to be similar to the cross-interaction layer in DCN, does not differentiate between the correct answer("eight") and the confusing answer("four").

%Another interesting takeaway is that the word interactions captured by DCN in layer 2, are similar to that of BERT after going through 7 layers of processing. Additionally, it is observed that in BERT, the role assumed by any layer changes across samples, thus making it further challenging to explain layer-wise functionality. 


